Nonlinear Equivalent Resistance-based Maximum Power Point Tracking (MPPT)

We present a nonlinear equivalent resistance tracking method to optimize the power output for solar arrays. Tracking an equivalent resistance results in nonlinear voltage step sizes in the gradient descent search loop. We introduce a new model for the combined solar module along with a DC-DC converter which results in a highly nonlinear dynamical system due to the inherent non-linearity of the PV cell topology and the switched DC-DC converter system. To guarantee stability over a range of possible operating regimes, we utilize a feedback linearization control approach to exponentially converge to the setpoint. Simulations are presented to illustrate the performance and robustness of the proposed technique.

==> Asymptotics_PESA.tex <==

% The computation time and scalability is optimized by utilizing a combination of semi-analytical methods from perturbation theory and numerical techniques including an efficient interpolation scheme for the solution of the Lambertian function.  

%\textbf{Lambert W-Function and PV Diode Models: }
%\label{SEC:Lambert}
%The proposed simulation engine leverages asymptotic series approximations to the following trancendental algebraic equations:
%\be
%\label{EQ:mainPertEQ}
%y = d_0 -d_1e^{\a_1 y} + \eps\left(d_2-d_3e^{\a_2 y}\right)
%\ee 
%and
%\be
%\label{EQ:lambertMain}
%we^{w} = z
%\ee
%where $d_i \in \R$ for $i\in[0,3]$ and $r\in\R$.  The two-diode model given in (\ref{EQ:TwoDiodeMain}) can be written in the form of (\ref{EQ:mainPertEQ}) where $y$ could be either current or voltage.  This is discussed below.  The solution to equation (\ref{EQ:lambertMain}) has been termed the Lambert-W function\footnote{The use of the letter \lq W\rq\ stems from its initial implementation in Maple in which the authors \cite{Corless_Gonnet_Hare_Jeffrey_1993} recognize the the work of \textbf{W}right on nonlinear delay differential equations \cite{Wright:1949,Wright:1955}.}, coined by Corless et al., in deference to Johann Heinrich Lambert (1728-1777) who solved the following trinomial algebraic equation \cite{Lambert:1758,Lambert:1772}:
%\bes
%y = q+y^m
%\ees
%Leonhard Euler (1707 �- 1783) transformed the above equation using: $y = z^{-\beta}$, $m = \frac{\a}{\beta}$, and %$q = (\a-\beta)v$ to get: 
%\bes
%z^{\a}-z^{\beta} = (\a-\beta)vz^{\a+\beta}
%\ees
%Dividing both sides by $\a-\beta$ and taking the limit as $\beta\rightarrow \a$ we get: 
%\bes
%we^{w} = x
%\ees
%where $w = -vz$ and $x = -v$.  

%We shall denote the solution of (\ref{EQ:lambertMain}) as $W(z)$ and refer to it informally as the \lq Lambert-W\rq function.  

%\textbf{Recasting the solution in terms of the Lambert W-Function}
%The Lambert-W function has proved useful in a variety of fields and applications including stability analysis of delay differential equations \cite{Chen_Moore_2002}, model combustion, enzyme kinematics, and analysis of algorithms \cite{Corless_Gonnet_Hare_Jeffrey_Knuth_1996}.  
%\ni \textit{Ideal One-Diode:} For the ideal one-diode model (\ref{EQ:oneDiodeIdeal1}), the current is expressed in closed form a function of the voltage since the right hand side of (\ref{EQ:oneDiodeIdeal1}) does not depend on $I$.  Hence, there is no need to employ the Lambert W-function.  To compute the power output, we have (using (\ref{EQ:oneDiodeIdeal1}))
%\be
%\label{EQ:oneDiodeMax}
%P = IV = V\left(I_{ph} - I_0\left(e^{\frac{V}{V_T}}-1\right)\right)
%\ee

%The maximum power point (MPP) can be found by finding the stationary points of (\ref{EQ:oneDiodeMax}).  We have 
%\bes
%\frac{\p P}{\p V} = I_{ph} + I_{01}-I_{01}e^{\frac{V}{V_{T}}}\left(1+\frac{V}{V_{T}}\right)
%\ees
%Setting the above expression to zero and defining $w = 1+\frac{V}{V_T}$, we arrive at 
%\bes
%we^w  = z
%\ees
%which is (\ref{EQ:lambertMain}) where
%where,
%\bes
%z = \frac{I_{ph}+I_{01}}{I_{01}}
%\ees
%Thus, the MPP voltage for the one-diode model can be found by the Lambert-W function and setting $V^{*} = (W-1)V_T$.  The maximum power is obtained by
%\bes
%P^* = V^*\left(I_{ph} - I_0\left(e^{\frac{V^*}{V_T}}-1\right)\right)
%\ees
%In summary, in the ideal one-diode model case, both $I$ and $V$ can be expressed in closed form as analytical functions of $V$ and $I$, respectively. 
%The equation for the maximum voltage operating point can be expressed in the form of (\ref{EQ:lambertMain}).  

%\ni \textit{One-Diode with Series and Shunt Resistances:}  As mentioned above, the first use of the Lambert-W function to solve a PV diode equation was given by Petrone \emph{et al}. \cite{Petrone:2007}.  The model used is obtained by setting $I_{02} = 0$ in (\ref{EQ:TwoDiodeMain})
%\be
%\label{EQ:OneDiodeWithRsRsh}
%I = I_{ph} - I_{01}\left(e^{\frac{(V+R_s I)}{V_{T_1}}}-1\right)-\frac{V+IR_s}{R_{sh}}
%\ee
%We can express the above more succinctly as
%\be
%\label{EQ:genericOneDiodeForm}
%y = d_0-d_1 e^{\a_1 y}
%\ee
%where $y = I $ and
%\bea
%\label{EQ:paramsOneDiodeI}
%d_0 &=& r_0^{-1}\left(I_{ph}-\frac{V}{R_{sh}+I_{01}}\right)\\
%r_0 &=& 1+\frac{R_s}{R_{sh}}\\
%d_1 &=& r_0^{-1}I_{01}e^{\frac{V}{V_{T_1}}}\\
%\a_1&=&\frac{R_s}{V_{T_1}}
%\eea
%We can transform (\ref{EQ:genericOneDiodeForm}) to 
%\bes
%we^{w} = x
%\ees
%where 
%\beas
%w &=& \a_1 d_0-\a_1y\\
%x &=& \a_1d_1e^{\a_1d_0}
%\eeas
%Using the Lambert-W function we can obtain closed-form solutions for $y=I$ or $y = V$ as %follows: 
%\be
%y = \frac{1}{\a_1}\left(\a_1 d_0 -W(x)\right)
%\ee

==> Background_PESA.tex <==
\subsection{Solar Modeling}
In the simplest representation, a PV cell is assumed to be a superposition of the dark and illuminated current-voltage characteristics.  This assumption leads to the \emph{ ideal one-diode} model related current (I) to voltage (V) given by
\be
\label{EQ:oneDiodeIdeal1}
I = I_{ph} - I_0\left(e^{\frac{qV}{kT}}-1\right)
\ee
where $I_{ph}$(A) denotes the photo-generated current, $I_0$(A) denotes the dark saturation current, $q$(Coulombs) denotes the electric charge carried by a single photon, $k$ denotes the Boltzmann constant ($J\cdot K^{-1}$), and $T$ denotes the cell temperature ($K$).  

\emph{Open Circuit Voltage: }
At the open-circuit operating point, we have $I = 0$.  Denoting the voltage at this point by $V_{oc}$ we find: 
\bes
V_{oc} = V_T\ln\left(1+\frac{I_{ph}}{I_{0}}\right)
\ees
where $V_T \eqd \frac{kT}{q}$ is the thermal voltage.  


\emph{Short Circuit Current: }At the short-circuit operating point, we have $V = 0$.  Denoting the current at this point by $I_{sc}$ we find: 
\bes
I_{sc} = I_{ph}
\ees
 
The ideal one-diode model has several shortcomings including limited characterization of two-dimesional current flow, surface recombination, ligh confinement, back-surface field, and others \cite{CastanerBook:2002}.  Furthermore, resistive losses stemming from semiconductor resistivity, contact resistance, and parallel losses accross the junction due to partial short circuits are not taken into account.  To address these limitations, the one-diode (\ref{EQ:OneDiodeMain}) or two-diode (\ref{EQ:TwoDiodeMain}) model can be used:

\be
\label{EQ:OneDiodeMain}
I = I_{ph} - I_{01}\left(e^{\frac{q(V+R_s I)}{n_1 kT}}-1\right)-\frac{V+IR_s}{R_{sh}}
\ee

\bea
\label{EQ:TwoDiodeMain}
I &=& I_{ph} - I_{01}\left(e^{\frac{q(V+R_s I)}{n_1 kT}}-1\right)- I_{02}\left(e^{\frac{q(V+R_s I)}{kT}}-1\right)\nonumber \\
&&-\frac{V+IR_s}{R_{sh}}
\eea
where $I_{01}$, denotes the dark saturation current of diffusion diode (A), $I_{02}$ denotes the dark saturation current of recombination diode (A), $R_s$ denotes the series resistance ($\Omega$), $R_{sh}$ denotes the shunt resistance ($\Omega$), and $n_i$ denotes the ideality factors (\textit{non-dimensional}).  For the one- and two- diode models which include ideality factors we shall sometimes use the expression for the thermal voltage $V_{T_i} \eqd \frac{n_i kT}{q}$.  In our simulations presented in the last section, however, we set both ideality factors to unity.   The key points of the two diode model are summarized as follows: 
\begin{description}
\item[Series Resistance]\hfill\\
Current generated by incoming photons travel through resistive semiconductor material in both the base and emitter regions.  Furthermore, resistive losses occur due to the contacts, metal grid, and current colloecting bus. 
\item[Shunt Resistance]\hfill\\
This term models parallel losses due to localized short circuits in the emitter layer.  These losses are primarily due to the manufacturing compromises that arise in the mass fabrication of PV cells and modules.   
\item[Diffusion Diode]\hfill\\
The diffusion diode (first exponential term in (\ref{EQ:TwoDiodeMain})) sometimes requires a \emph{non-ideality} factor in order to fit real data.  This factor is termed, $n_1$.  
\item[Recombination Diode]\hfill\\
The recombination diode (second exponential term in (\ref{EQ:TwoDiodeMain})) is appended to model non-ohmic current paths in parallel with the photodiode.  It also includes a \emph{non-ideality} factor termed, $n_2$.  
\end{description}



==> LambertApproximation.tex <==

In this section we describe our approach for rapid asymptotic approximation of the Lambert-W function used in the previous sections.  We begin with some prelinary defintions.  


Let $\R$ denotes the set of real numbers, $\Z$ the set of integers, and $\Z^+$ the set of non-negative integers.
\begin{definition}
Let $f,g: [0,\eps_0) \rightarrow \R$.  We write $f = \O(g)$ as $\eps \downarrow 0$ if and only if there exists real constants $c>0$ and $\eps_1>0$ such that
\bes
|f(\eps)| \leq c|g(\eps)|
\ees
for all $\eps \in (0,\eps_1)$.   

\end{definition}
\begin{definition}
Let $f,g: [0,\eps_0) \rightarrow \R$.  We write $f = \o(g)$ as $\eps \downarrow 0$ if and only if for \emph{any} $\delta >0$ there exists  a real constant $\eps_1>0$ such that
\bes
|f(\eps)| \leq \delta|g(\eps)|
\ees
for all $\eps \in (0,\eps_1)$.  
\end{definition}
Let $\{\phi_{i}\}$ be a collection of $N$ real-valued functions: 
\bes
\phi_i: [0,\eps_0) \rightarrow \R
\ees
where $i\in[1,N]$ and $\eps_0 >0.$  \\



\begin{definition}
$\{\phi_{i}\}_{i = 1}^{N}$ is said to be an asymptotic sequence if and only if $\phi_{i+1} = \o(\phi_i)$ for any $i\in[1,N-1]$ as $\eps \downarrow 0$.  
\end{definition}
The idea of an asymptotic sequence is, loosely speaking, that each additional term added is \lq less important\rq\ in the sense that it tends to zero faster than the previous term.  We have the following useful lemma:  
\begin{lemma}
Let $\{\phi_{i}(\eps)\}_{i = 1}^{N}$ denote an aysmptotic sequence of $N$ terms where each $\phi_i: (0,\eps^*]\rightarrow \R$.  Then, $\phi_n = \o(\phi_m)$ as $\eps \downarrow 0$ for any $1 \leq m < n \leq N$.  
\end{lemma}
\proof
Define $s= n-m\geq 1$.  Then, 
\bes
\left|\frac{\phi_n}{\phi_m}\right| = \left|\frac{\phi_n}{\phi_{n-1}}\cdot \frac{\phi_{n-1}}{\phi_{n-2}}\cdots \frac{\phi_{n-s+1}}{\phi_{m}}\right|
\ees
For any $k\in[0,s-1]$ and $\del_k>0$, there exists an $\eps_k\in(0,\eps^*)$ such that 
\bes
\left|\frac{\phi_{n-k}}{\phi_{n-k-1}}\right| \leq \del_k
\ees
Hence, 
\bes
\left|\frac{\phi_{n}}{\phi_{m}}\right| \leq \del_0\cdot \del_1 \cdots \del_{s-1}\;\;\; \forall \eps \in (0,\min(\eps_0,\eps_1,\ldots,\eps_{s-1})
\ees
\endproof

When \lq plugging\rq\ an asymptotic series approximation into an algebraic or differential equation, various combinations of the terms of the asymptotic sequence result.  For example, polynomials in the unknown solution would result in polynomials in the terms of the asymptotic sequence.  While the relative ordering of the asymptotic sequence is known, by definition, it is essential to determine the relative ordering of the terms due to such nonlinear mappings.  We have the following lemma which is used below:   
\begin{lemma}
Let $\{\phi_i\}_{i = 1}^{N}$ denote an $N$-term asymptotic sequence.  Let $\a,\beta \in\R^N$ be multi-indices.  Then, 
\bes
\phi^\beta =\o(\phi^{\a})
\ees
if 
\bes
???????????????\prod_{i=1}^N i^{\beta_i} > \prod_{i=1}^N i^{\a_i}???????????????
\ees
where $\phi^{\beta} = \phi_1^{\beta_1}\cdot \phi_2^{\beta_2}\cdots \phi_N^{\beta_N}$ and  $\phi^{\a} = \phi_1^{\a_1}\cdot \phi_2^{\a_2}\cdots \phi_N^{\a_N}$ 
\end{lemma}

The above lemma is rather weak.  The difficulty in strengthening it can be easily seen by considering the following two example asymptotic sequences: $\{\phi_i\}$ and $\{\psi_i\}$ where
\bes
\phi_i = \eps^{i}\;\;\;i\in[1,N]
\ees
and
\bes
\ba{lll}
\psi_1 &=& \ln(\eps^{-1})\\
\psi_2 &=& \ln\left(\ln(\eps^{-1})\right)^s\\
\psi_3 &=& \ln\left(\ln(\eps^{-1})\right)\\
\psi_4 &=& \ds \frac{\ln\left(\ln(\eps^{-1})\right)^{p}}{\ln(\eps^{-1})}\\
\psi_5 &=& \ds \frac{\ln\left(\ln(\eps^{-1})\right)^{p-1}}{\ln(\eps^{-1})}\\
\psi_6 &=& \ds \frac{\ln\left(\ln(\eps^{-1})\right)^{r}}{\ln(\eps^{-1})^2}
\ea
\ees
where $s>1$, and $r,p$ are any integers.  The sequence $\{\phi_i\}$ is clearly asymptotic since: 
\bes
\frac{\phi_n}{\phi_m} = \eps^{n-m} \rightarrow 0 \;\mbox{as } \eps\downarrow 0\mbox{ for } n>m
\ees
Furthermore, we have $\phi^{\beta} = \o(\phi^{\a})$ if and only if
\be
\label{EQ:exampleOrdering1}
\prod \beta_i \cdot i > \prod \a_i \cdot i
\ee 
for any multi-indices, $\a$ and $\beta$.  

To show the sequence $\{\psi_i\}$ is well-ordered\footnote{The term, \emph{well-ordered}, is understood to be synomynous with \emph{asymptotic} in the discusion of sequences.} we need the following lemma: 

\begin{lemma}
\label{LEMMA:ordering1}
\bes
\left(\ln\left(\ln(\eps^{-1})\right)\right)^p = \o\left(\ln(\eps^{-1})\right)^q
\ees
for any $p\in \Z$ and any $q\in\Z^{+}$.
\end{lemma}
\proof
If $\p\leq 1$, then the result follows trivially.  For $p>1$, we have 
\bes
\frac{\frac{d}{d\eps}\left(\ln(\ln(\eps^{-1}))\right)^p}{\frac{d}{d\eps}\left(\ln(\eps^{-1})\right)^q} = \frac{p\left(\ln(\ln(\eps^{-1}))\right)^{p-1}}{q\left(\ln(\eps^{-1})\right)^q}
\ees
Differentiating $k$ times we have: 
\bes
\frac{\frac{d^k}{d\eps^k}\left(\ln(\ln(\eps^{-1}))\right)^p}{\frac{d}{d\eps}\left(\ln(\eps^{-1})\right)^q} = \frac{p(p-1)\cdots(p-k+1)\left(\ln(\ln(\eps^{-1}))\right)^{p-k}}{q^k\left(\ln(\eps^{-1})\right)^q}
\ees
Setting $k = p$, and using $L'Hopital's$ rule we have
\bes
\lim_{\eps \rightarrow 0^+} \frac{\left(\ln(\ln(\eps^{-1}))\right)^p}{\left(\ln(\eps^{-1})\right)^q}  = \lim_{\eps \rightarrow 0^+} \frac{p!}{q^{p}(\ln(\eps^{-1}))^q} = 0
\ees
\endproof
Hence, it follows that: 
\beas
\lim_{\eps\rightarrow 0^+}\frac{\psi_2}{\psi_1} &=& \lim_{\eps\rightarrow 0^+}\frac{\ln\left(\ln(\eps^{-1})\right)^s}{\ln(\eps^{-1})} = 0\\
\lim_{\eps\rightarrow 0^+}\frac{\psi_3}{\psi_2} &=& \lim_{\eps\rightarrow 0^+}\frac{1}{\ln(\ln(\eps^{-1}))^{s-1}} = 0\\
\lim_{\eps\rightarrow 0^+}\frac{\psi_4}{\psi_3} &=& \lim_{\eps\rightarrow 0^+}\frac{\ln\left(\ln(\eps^{-1})\right)^{p-1}}{\ln(\eps)} = 0\\
\lim_{\eps\rightarrow 0^+}\frac{\psi_5}{\psi_4} &=& \lim_{\eps\rightarrow 0^+}\frac{1}{\ln\ln((\eps))} = 0\\
\lim_{\eps\rightarrow 0^+}\frac{\psi_6}{\psi_5} &=& \lim_{\eps\rightarrow 0^+}\frac{\ln\left(\ln(\eps^{-1})\right)^{r-p+1}}{\ln(\eps)} = 0
\eeas

 
Consider terms generated by $\left(\sum_{i = 1}^{6}\psi_i\right)^2$.  Using Lemma \ref{LEMMA:ordering1}, we find
\bea
\psi_2^2 &=& \o(\psi_1\psi_3)\\
\psi_3^{2} &=& \o(\psi_4 \psi_1) \mbox{ if } p>1\nn\\
\psi_4 \psi_1&=& \o(\psi_3^{2}) \mbox{ if } p\leq 1\\
\psi_4 \psi_2&=& \o(\psi_3^2)
\eea
Clearly the above violates ordering conditions given in (\ref{EQ:exampleOrdering1}).  









Lastly, we define what we mean by an asymptotic series approximation.  

\begin{definition}
Let $f,g: [0,\eps_0) \rightarrow \R$.  The function $g$ is said to be an asymptotic approximation of $f$ if and only if
\bes
f-g = \o(g)
\ees
as $\eps \downarrow 0$.  
\end{definition}

\begin{definition}
Let $f,\phi_i: [0,\eps_0) \rightarrow \R$ for $i\in [1,N]$.  Then the sum $\sum_{i=1}^{N}\phi_i$ is said to be an $N$-term asymptotic series approximation to $f$ if and only if $\{\phi_{i}\}_{i = 1}^{N}$ is an asymptotic sequence and 
\bes
f-\sum_{i=1}^{N}\phi_i = \o(\phi_N)
\ees
as $\eps \downarrow 0$. 
\end{definition}





\subsubsection{The Approach}
Let $\{\phi_{i}(\nu)\}_{i = 1}^{N}$ denote an aysmptotic sequence as\footnote{For the remainder of this note, we shall omit the explicit statement $\nu \downarrow 0$ which appends asymptotic function related definitions.} $\nu \downarrow 0$.  A quick sketch of (\ref{EQ:main0}) reveals that there exists only one (positive) solution for $\nu >0$.  Furthermore, $\left.\frac{e^{-x}}{x}\right|_{x = \ln(\nu^{-1})} = \frac{\nu}{\ln(\nu^{-1})} < \nu$ if $\nu <e^{-1}$.  Hence, the solution lies to the left of $\ln(\nu^{-1})$.  Taking the $\ln(\cdot)$ of both sides of (\ref{EQ:main0}) we get: 
\bes
x = \ln(\nu^{-1})-\ln(x)=: T(x)
\ees
Hence, the solution is a fixed point of the operator, $T(\cdot)$.  On the interval $(\ln(\nu^{-1}),\infty)$, $T$ is a contraction since the norm of its gradient is less than unity\footnote{This can be proved by the mean-value theorem.}.  Hence, by the contraction mapping principle, the sequence of real numbers $x_{k+1} := T(x_k)$ for $k = 1,2,\ldots$  converges to a unique fixed point $x^{*}$.  Setting the initial solution to $x_1 = \ln(\nu^{-1})$ we get
\bes
x_2 = \ln(\nu^{-1})-\ln\left(\ln(\nu^{-1})\right)
\ees
It is here we depart the iterative approach and turn to asymptotic analysis.  That is, we seek an asymptotic approximation to the solution of (\ref{EQ:main0}) given by
\be
\label{EQ:xGeneral}
x = \sum_{i = 1}^{N} \phi_i(\nu) + \o(\phi_N(\nu))
\ee
Substitution of (\ref{EQ:xGeneral}) into (\ref{EQ:main0}) and Taylor expanding the left hand side about $y_0>0$ we get: 
\be
\label{EQ:expansion1}
\ba{l}
\ds e^{-y_0}\left(1-\left(\sum_{i=1}^{N} \phi_i - y_0 + \o(\phi_N)\right) + \frac{1}{2}\left(\sum_{i=1}^{N} \phi_i - y_0 + \o(\phi_N)\right)^2\right.\\
\left.-\frac{1}{6}\left(\sum_{i=1}^{N} \phi_i - y_0 + \o(\phi_N)\right)^3\right) + R\\
= \ds \nu\left(\sum_{i = 1}^{N} \phi_i(\nu) + \o(\phi_N(\nu))\right)
\ea
\ee

Define
\be
\phi_1(\nu) = \ln(\nu^{-1})
\ee
and
\be
\phi_2(\nu) = \ln\left(\frac{1}{\ln(\nu^{-1})}\right)
\ee
We note that $\{\phi_1,\phi_2\}$ is well-ordered since
\bes
\lim_{\nu\rightarrow 0^+} \left|\frac{-\ln\left(\ln(\nu^{-1})\right)}{\ln(\nu^{-1})}\right| = 0
\ees
by Lemma \ref{LEMMA:ordering1}.   

Next, we choose the point to be Taylor expanded about to be $y_0 = \phi_1 + \phi_2 = \ln\left(\frac{\nu^{-1}}{\ln(\nu^{-1})}\right)$.  Substitution of $y_0$ into (\ref{EQ:expansion1}) and setting $N = 6$ we get: 
\be
\ba{l}
\nu \ln(\nu^{-1})\left(\overbrace{1}^{\mbox{\textcircled{\scriptsize{1}}}}-\left(\overbrace{\phi_3}^{\mbox{\textcircled{\scriptsize{2}}}}+\overbrace{\phi_4}^{\mbox{\textcircled{\scriptsize{3}}}}+\overbrace{\phi_5}^{\mbox{\textcircled{\scriptsize{4}}}}+\overbrace{\phi_6}^{\mbox{\textcircled{\scriptsize{5}}}}+\o(\phi_6)\right)\right.\\ \frac{1}{2}\left(\overbrace{\phi_3^2}^{\mbox{\textcircled{\scriptsize{a}}}}+\overbrace{2\phi_3\phi_4}^{\mbox{\textcircled{\scriptsize{b}}}}+\overbrace{2\phi_3\phi_5}^{\mbox{\textcircled{\scriptsize{c}}}}+\overbrace{\phi_4^2}^{\mbox{\textcircled{\scriptsize{d}}}} + \o(\phi_3\phi_5)\right)\\
-\frac{1}{6}\left(\overbrace{\phi_3^3}^{\mbox{\textcircled{\scriptsize{i}}}}+\overbrace{3\phi_3^2\phi_4}^{\mbox{\textcircled{\scriptsize{ii}}}} + \o(\phi_3^2\phi_4)\right)+ R\\
= \nu \left(\underbrace{\phi_1}_{\mbox{\textcircled{\scriptsize{1'}}}}+\underbrace{\phi_2}_{\mbox{\textcircled{\scriptsize{2'}}}}+\underbrace{\phi_3}_{\mbox{\textcircled{\scriptsize{3'}}}}+\underbrace{\phi_4}_{\mbox{\textcircled{\scriptsize{4'}}}}+\underbrace{\phi_5}_{\mbox{\textcircled{\scriptsize{5'}}}}+\o(\phi_5)\right)
\ea
\ee

\textbf{Balancing: }\\
Term \textcircled{\scriptsize{1}} balances with \textcircled{\scriptsize{1'}} since $\phi_1 = \ln(\nu^{-1})$.  Term \textcircled{\scriptsize{2}} balances with \textcircled{\scriptsize{2'}} if
\bes
\phi_3 = \frac{\ln(\ln(\nu^{-1}))}{\ln(\nu^{-1})}
\ees
The sequence $\{\phi_1,\phi_2,\phi_3\}$ is well-ordered since $\frac{\phi_3}{\phi_2} = \frac{-1}{\ln(\nu^{-1})}\rightarrow 0$.  

Term \textcircled{\scriptsize{a}} and \textcircled{\scriptsize{3}} balance with \textcircled{\scriptsize{3'}} if
\be
\phi_4 = -\frac{\phi_3}{\ln(\nu^{-1})} + \frac{1}{2}\phi_3^2
\ee
The sequence $\{\phi_1,\phi_2,\phi_3,\phi_4\}$ is well-ordered since $\frac{\phi_4}{\phi_3} = \frac{-1}{\ln(\nu^{-1})}+\frac{1}{2}\phi_3\rightarrow 0$.  

Before continuing note that $\phi_3\phi_4 = \o(\phi_3^2)$ since $\frac{\phi_3\phi_4}{\phi_3^2} = -\frac{1}{\ln(\ln(\nu^{-1}))} + \frac{1}{2} \rightarrow \frac{1}{2} \neq 0$.  Note this cleary violates (\ref{}).  

Terms \textcircled{\scriptsize{4}}, \textcircled{\scriptsize{b}}, and \textcircled{\scriptsize{i}} balance with \textcircled{\scriptsize{4'}} if
\be
\phi_5 = \phi_4\phi_4 -\frac{1}{6}\phi_3^3 -\frac{\phi_4}{\ln(\nu^{-1})}
\ee
The sequence $\{\phi_1,\phi_2,\phi_3,\phi_4,\phi_5\}$ is well-ordered since 
\bes
\frac{\phi_5}{\phi_4}  = \phi_3-\frac{1}{6}\left(\frac{\phi_3}{-\frac{1}{\ln(\nu^{-1})\phi_3}+\frac{1}{2}}\right)-\frac{1}{\ln(\nu^{-1})}\rightarrow 0
\ees
By further application of Lemma \ref{LEMMA:ordering1} we find that $\phi_4^2 = \O(\phi_3\phi_5)$ and $\phi_4^2 = \O(\phi_3^2\phi_4)$.  Hence, it follows that terms \textcircled{\scriptsize{5}}, \textcircled{\scriptsize{c}}, \textcircled{\scriptsize{d}},and \textcircled{\scriptsize{ii}} balance with \textcircled{\scriptsize{5'}} if
\be
\phi_6 = \frac{1}{2}\left(2\phi_3\phi_5 + \phi_4^2\right) -\frac{1}{2}\phi_3^{2}\phi_4 -\frac{\phi_5}{\ln(\nu^{-1})}
\ee

\be
\phi_1(\nu) = \ln(\nu^{-1})
\ee
and
\be
\phi_2(\nu) = \ln\left(\frac{1}{\ln(\nu^{-1})}\right)
\ee
\beas
\phi_1(\nu) &=& \ln(\nu^{-1})\\
\phi_2(\nu) &=& \ln\left(\frac{1}{\ln(\nu^{-1})}\right)\\
\phi_3 &=& \frac{\ln(\ln(\nu^{-1}))}{\ln(\nu^{-1})}\\
\phi_4 &=& -\frac{\phi_3}{\ln(\nu^{-1})} + \frac{1}{2}\phi_3^2\\
\phi_5 &=& \phi_4\phi_4 -\frac{1}{6}\phi_3^3 -\frac{\phi_4}{\ln(\nu^{-1})}\\
\phi_6 &=& \frac{1}{2}\left(2\phi_3\phi_5 + \phi_4^2\right) -\frac{1}{2}\phi_3^{2}\phi_4 -\frac{\phi_5}{\ln(\nu^{-1})}
\eeas
     

 \begin{figure*}[t]
\begin{center}
\epsfig{figure=ErrorVsSolutionNumber.eps,scale=0.6}
\end{center}
\caption{Approximation Error versus Number of Terms: On the left hand side $\eps = 0.3$ and on the right hand side $\eps = 0.1$.  The approximation error is defined by $|x-x_i|$ where $x_i = \sum_{k = 1}^{i} \phi_k$}
\label{FIG:ErrorVsSolutionNumber}
\end{figure*}

\begin{figure}[t]
\begin{center}
\epsfig{figure=ErrorVsEps.eps,scale=0.6}
\end{center}
\caption{Approximation Error versus $\eps$:  The approximation error is defined by $|x-x_i|$ where $x_i = \sum_{k = 1}^{i} \phi_k$}
\label{FIG:ErrorVsEps}
\end{figure}
